A Theoretical Explanation of Activation Sparsity through Flat Minima and Adversarial Robustness

A recent empirical observation (Li et al., 2022b) of activation sparsity in MLP blocks offers an opportunity to drastically reduce computation costs for free. Although having attributed it to training dynamics, existing theoretical explanations of activation sparsity are restricted to shallow networks, small training steps and special training, despite its emergence in deep models standardly trained for a large number of steps. To fill these gaps, we propose the notion of gradient sparsity as one source of activation sparsity and a theoretical explanation based on it that sees sparsity a necessary step to adversarial robustness w.r.t. hidden features and parameters, which is approximately the flatness of minima for well-learned models. The theory applies to standardly trained LayerNorm-ed MLPs, and further to Transformers or other architectures trained with weight noises. Eliminating other sources of flatness except for sparsity, we discover the phenomenon that the ratio between the largest and smallest non-zero singular values of weight matrices is small. When discussing the emergence of this spectral concentration, we use random matrix theory (RMT) as a powerful tool to analyze stochastic gradient noises. Validational experiments are conducted to verify our gradient-sparsity-based explanation. We propose two plug-and-play modules for both training and finetuning for sparsity. Experiments on ImageNet-1k and C4 demonstrate their 50% sparsity improvements, indicating further potential cost reduction in both training and inference.

==> defs.tex <==
\makeatletter
\newenvironment{breakablealgorithm}
  {% \begin{breakablealgorithm}
   \begin{center}
     \refstepcounter{algorithm}% New algorithm
     \hrule height.8pt depth0pt \kern2pt% \@fs@pre for \@fs@ruled
     \renewcommand{\caption}[2][\relax]{% Make a new \caption
       {\raggedright\textbf{\ALG@name~\thealgorithm} ##2\par}%
       \ifx\relax##1\relax % #1 is \relax
         \addcontentsline{loa}{algorithm}{\protect\numberline{\thealgorithm}##2}%
       \else % #1 is not \relax
         \addcontentsline{loa}{algorithm}{\protect\numberline{\thealgorithm}##1}%
       \fi
       \kern2pt\hrule\kern2pt
     }
  }{% \end{breakablealgorithm}
     \kern2pt\hrule\relax% \@fs@post for \@fs@ruled
   \end{center}
  }
\makeatother


\newcommand{\set}[1]{\{#1\}}
\newcommand{\setName}[1]{{\textbb{#1}}}
\newcommand{\floor}[1]{{\left\lfloor #1 \right\rfloor}}
\newcommand{\ceil}[1]{{\left\lceil #1 \right\rceil}}
\newcommand{\srt}[2]{{\texttt{#1}(#2)}}
\newcommand{\srtName}[1]{{\texttt{#1}}}
\newcommand{\nil}{{\textrm{NIL}}}
\newcommand{\gh}{{\mbox{-}}}
\newcommand{\seg}[3]{{#1[#2\dots#3]}}
\newcommand{\arr}[2]{{#1[#2]}}
% \newcommand{\interval}[2]{{\left[#1,#2\right]}}
\newcommand{\sqrket}[2]{{\left[#1,#2\right]}}
\newcommand{\angBracket}[1]{{\left\langle#1\right\rangle}}
\newcommand{\size}[1]{{\left|{#1}\right|}}
\newcommand{\abs}[1]{\size{#1}}
\newcommand{\mathCmt}[1]{{\text{(#1)}}}
\newcommand{\mn}[1]{{\min\set{#1}}}
\newcommand{\mx}[1]{{\max\set{#1}}}
\newcommand{\event}[1]{{\set{#1}}}
\newcommand{\bigO}[1]{{O\left(#1\right)}}
\newcommand{\bigTheta}[1]{{\Theta\left(#1\right)}}
\newcommand{\bigOmg}[1]{{\Omega\left(#1\right)}}
\newcommand{\diam}[1]{{\mathop{\mathrm{diam}}\left(#1\right)}}
\newcommand{\dfsWhite}{{\textrm{WHITE}}}
\newcommand{\dfsGray}{{\textrm{GRAY}}}
\newcommand{\dfsBlack}{{\textrm{BLACK}}}
\newcommand{\lcm}{{\mathop{\mathrm{lcm}}}}
\newcommand{\intGroup}[1]{{\mathbb{Z}_{#1}}}
\newcommand{\substitute}[2]{{\left[\frac{#1}{#2}\right]}}
\newcommand{\bvec}[1]{\mathbb{#1}}
\newcommand{\Null}{\textrm{Null}}
% \newcommand{\unit}[1]{{\,\,\mathrm{#1}}}
\newcommand{\mathsc}[1]{\text{\sc{#1}}}
\newcommand{\dom}{\mathrm{dom}}
\newcommand{\pr}[1]{{\mathrm{Pr}\left[#1\right]}}
\newcommand{\var}[1]{{\mathbf{Var}\left[{#1}\right]}}
% \newcommand{\fact}[1]{{{#1}!}}
\newcommand{\indic}[1]{{\mathrm{I}\left[{#1}\right]}}
\newcommand{\mathcomment}[1]{\text{(#1)}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\inlinecode}[1]{\texttt{#1}}
\newcommand{\cardinality}[1]{{\left|{#1}\right|}}
\newcommand{\argmin}{{\mathrm{argmin}}}
\newcommand{\funcmodify}[3]{{{#1}\left\{{#2} \leadsto {#3}\right\}}}
\newcommand{\sgn}{\textrm{sgn}}
\NewDocumentCommand{\reals}{}{\mathbb{R}}
\NewDocumentCommand{\nats}{}{\mathbb{N}}
\NewDocumentCommand{\complexes}{}{\mathbb{C}}
\NewDocumentCommand{\dd}{}{\mathrm{d}}
\NewDocumentCommand{\rpart}{m}{\mathrm{Re}\left(#1\right)}
\NewDocumentCommand{\ipart}{m}{\mathrm{Im}\left(#1\right)}

\DeclareMathOperator{\supportinner}{supp}

\NewDocumentCommand{\mset}{m}{\set{#1}}
\NewDocumentCommand{\opt}{O{}}{\mathrm{OPT}_{\mathrm{#1}}}
\NewDocumentCommand{\sol}{O{}}{\mathrm{SOL}_{\mathrm{#1}}}
\NewDocumentCommand{\support}{m}{\supportinner{#1}}
\NewDocumentCommand{\ex}{O{} m}{{\mathbf{E}_{#1}\left[#2\right]}}
\DeclareMathOperator{\rangeinner}{ran}
\NewDocumentCommand{\range}{m}{\rangeinner{#1}}
\NewDocumentCommand{\defeq}{}{\triangleq}
\NewDocumentCommand{\mutualinfo}{O{} O{} m m}{I_{#1}^{#2}(#3; #4)}
\NewDocumentCommand{\entropy}{O{} O{} m m}{H_{#1}^{#2}(#3)}
\NewDocumentCommand{\prob}{O{} O{} m}{\mathrm{P}^{#1}_{#2}\left[#3\right]}
\NewDocumentCommand{\transpose}{}{T}
\NewDocumentCommand{\trace}{m}{\mathrm{tr}\left(#1\right)}
\NewDocumentCommand{\hadamard}{}{\odot}
\NewDocumentCommand{\diag}{m}{\mathrm{diag}\left(#1\right)}
\NewDocumentCommand{\gaussian}{m m}{\mathcal{N}\left(#1, #2\right)}
\NewDocumentCommand{\chisquared}{m}{\chi^2_{#1}}

% define theorem-like environments
\newenvironment{cntrProofTree}{\begin{center}\begin{prooftree}}{\end{prooftree}\end{center}}
\DeclareMathOperator*{\argmax}{arg\,max}

% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}[theorem]{Lemma}
% \theoremsymbol{\ensuremath{\color{lightgray}\blacksquare}}
% \newtheorem*{proof}{Proof}

% \newtheorem{theorem}{Theorem}
% \newtheorem{corollary}{Corollary}
% \newtheorem{lemma}{Lemma}
% \newtheorem{definition}{Definition}
% \newtheorem{remark}{Remark}
% \newtheorem{observation}{Observation}
% \newtheorem{conjecture}{Conjecture}

\declaretheorem[name=Theorem]{thm}
\declaretheorem[name=Corollary]{restatablecorollary}


==> experiments/experiments.tex <==

\input{experiments/theoretical.tex}

==> failed/diagonal.tex <==
\subsubsection{Initial Diagonality of $\left(K^l \left(K^l\right)^\transpose\right) \hadamard M^l$}\label{sec:sparsity_at_initialization}

The Hadamard product forms an interesting structure in the sense that the simplicity of Hadamard product allows $K^l \left(K^l\right)^\transpose$ to shadow tedious details in $M^l$ of deeper layers. If we prove $K^l \left(K^l\right)^\transpose$ is very close to a diagonal matrix and $M^l$'s diagonal elements take moderate portions in the total (squared $L_2$) norm, we can conclude that $\left(K^l \left(K^l\right)^\transpose\right) \hadamard M^l$ is approximately diagonal.

Noting that $K^l \left(K^l\right)^\transpose = \begin{bmatrix}\inner{K^l_i}{K^l_j}\end{bmatrix}_{i, j}$, whose diagonal elements are $\inner{K^l_i}{K^l_i} = \norm{K^l_i}_2^2 \ge 0 (i \neq j)$, we need to prove $\inner{K^l_i}{K^l_j} \approx 0$ for $i \neq j$. This property can emerge from modern initialization where entries are initialized with mutually independent and centered distribution. \cref{lemma:KKT_diagonality_at_initialization} provides a precise formulation for this intuition based on ubiquitous initialization.
\begin{lemma}[Diagonality of $K^l \left(K^l\right)^\transpose$ at initialization]\label{lemma:KKT_diagonality_at_initialization}
    Let $K^l \in \reals^{n \times d}$ be a matrix initialized by (Gaussian) Xavier or Kaiming initialization, then for sufficiently large $d$, there is
    \begin{enumerate}
        \item $\inner{K^l_i}{K^l_i} = \norm{K^l_i}_2^2 \stackrel{\textrm{w.h.p.}}{\ge} 0.5 p$. When $d = 100$, the probability of violation is already approximately $6.95 \times 10^{-6}$, according to numerical computations;
        \item If $i \neq j$, then $\ex{\inner{K^l_i}{K^l_j}} = 0$;
        \item If $i \neq j$, then $\ex{\inner{K^l_i}{K^l_j}^2} = \var{\inner{K^l_i}{K^l_j}} = \frac{p}{d}$;
    \end{enumerate}
    where $p = \frac{p' d}{n + d}, p' \in \set{2, 4}$ depending on which initialization is used. 
\end{lemma}
The proof of it is rather tedious so we leave it in \cref{proof:kkt_diagonality_at_initialization}. From \cref{lemma:KKT_diagonality_at_initialization} we can see that despite there being only $n$ diagonal elements but $n(n-1)$ non-diagonal elements, non-diagonal elements take at most $2$ or $3$ times portions in squared $L_2$ norm of the matrix than diagonal ones. This indicates that $K^l \left(K^l\right)^\transpose$ is approximately diagonal.

Now we show that $M^l$ is not too anti-diagonal in \cref{lemma:ml_diagonality}
\begin{lemma}[Diagonality of $M^l$]\label{lemma:ml_diagonality}
    Let $M^l \in \reals^{n \times n}$ be a symmetric, positive semi-definite matrix whose rank is at most $1$, as concluded in \cref{lemma:adversarial_and_sparsity} and \cref{theorem:main}. Then the diagonal elements are responsible for a portion at least $\frac{1}{n}$ in the total squared $L_2$ norm of $M^l$.
    \begin{proof}
        \cref{lemma:adversarial_and_sparsity} concluded that symmetric positive semi-definite $M^l$'s rank is at most $1$, so it can be decomposed into
        \begin{align}
            M^l = \lambda_1 m m^\transpose,
        \end{align}
        where $\lambda_1 \ge 0$ is the largest eigenvalue and $m$ is the corresponding normalized eigenvector.

        To measure how diagonal $M^l$ is, we compute the squared $L_2$ norm ratio between diagonal and all elements, i.e.
        \begin{align}
            r 
            \defeq& \frac{\trace{M^l \hadamard M^l}}{\trace{\left(M^l\right)^\transpose M^l}}\\
            =&  \frac{\trace{M^l \hadamard M^l}}{\lambda_1^2}.
        \end{align}
        Imitating \citet{hadamard_and_eigenvector}, there is
        \begin{align}
            M^l \hadamard M^l
            =&  \lambda_1^2 (m m^\transpose) \hadamard (m m^\transpose)\\
            =&  \lambda_1^2 (m \hadamard m) (m \hadamard m)^\transpose,
        \end{align}
        which leads to
        \begin{align}
            \trace{M^l \hadamard M^l}
            =&  \lambda_1^2 \trace{(m \hadamard m) (m \hadamard m)^\transpose} = \lambda_1^2 \norm{m \hadamard m}_2^2.
        \end{align}
        Therefore the norm ratio is
        \begin{align}
            r = \norm{m \hadamard m}_2^2.
        \end{align}
        The worst case, under the constraint that $\norm{m} = 1$, is $m = \begin{bmatrix} \frac{1}{\sqrt{n}}\end{bmatrix}_i$, which makes $r = \frac{1}{n}$.
    \end{proof}
\end{lemma}
\cref{lemma:ml_diagonality} indicates that the contribution to squared $L_2$ norms is quite uniform in $M^l$ and it is not the case that diagonal elements are adversarially small.

\begin{theorem}[Diagonality at initialization.]\label{theorem:diagonality_at_initialization}
    If $K^l \in \reals^{n \times d}$ is Xavier- or Kaiming-initialized, at initialization, the ratio of expected sqaured $L_2$ norms in $\left(K^l \left(K^l\right)^\transpose\right) \hadamard M^l$ between diagonal and all elements is at least
    \begin{align}
        \frac{0.4 d}{p n + 0.4 d - p} = \frac{0.4}{p' \frac{1 - 1/n}{1 + d /n} + 0.4}
    \end{align}
    when $d$ is sufficiently large, e.g. $d > 100$, where $p = \frac{p' d}{n + d}, p' \in \set{2, 4}$ depending on which initialization is used.
    \begin{proof}
        For entry at $(i, j)$, there is
        \begin{align}
            \ex{\left(\left(K^l \left(K^l\right)^\transpose\right) \hadamard M^l\right)_{i, j}^2}
            =&  \ex{\inner{K^l_i}{K^l_j}^2} \cdot \left(M^l_{i, j}\right)^2 
        \end{align}
        For diagonal elements, $\inner{K^l_i}{K^l_i} \ge 0$ and with w.h.p. $\inner{K^l_i}{K^l_i} > 0.5$ by \cref{lemma:KKT_diagonality_at_initialization}. Therefore for diagonal elements there is
        \begin{align}
            \ex{\sum_{i} \left(\left(K^l \left(K^l\right)^\transpose\right) \hadamard M^l\right)_{i, i}^2}
            =&  \sum_{i} \ex{\inner{K^l_i}{K^l_i}^2} \cdot \left(M^l_{i, i}\right)^2 \\
            \ge&\sum_{i} 0.4 \cdot \left(M^l_{i, i}\right)^2 = 0.4 \cdot \trace{M^l \hadamard M^l},
        \end{align}
        given that $d$ is sufficiently large, e.g. $d > 100$.

        The expected sum of squared non-diagonal elements is
        \begin{align}
            \ex{\sum_{i \neq j} \left(\left(K^l \left(K^l\right)^\transpose\right) \hadamard M^l\right)_{i, j}^2}
            =&  \sum_{i \neq j} \ex{\inner{K^l_i}{K^l_j}^2} \cdot \left(M^l_{i, j}\right)^2\\
            =&  \sum_{i \neq j} \frac{p}{d} \left(M^l_{i, j}\right)^2 & \left(\text{\cref{lemma:KKT_diagonality_at_initialization}}\right)\\
            =&  \frac{p}{d} \left(\trace{\left(M^l\right)^\transpose M^l} - \trace{M^l \hadamard M^l}\right)
        \end{align}
        The ratio of expected squared $L_2$ norms between diagonal and all elements is
        \begin{align}
            &\frac{\ex{\sum_{i} \left(\left(K^l \left(K^l\right)^\transpose\right) \hadamard M^l\right)_{i, i}^2}}{\ex{\sum_{i, j} \left(\left(K^l \left(K^l\right)^\transpose\right) \hadamard M^l\right)_{i, j}^2}}\\
            \ge&    \frac{0.4 \cdot \trace{M^l \hadamard M^l}}{\frac{p}{d} \left(\trace{\left(M^l\right)^\transpose M^l} - \trace{M^l \hadamard M^l}\right) + 0.4 \cdot \trace{M^l \hadamard M^l}}\\
            =&  \frac{0.4 r}{\frac{p}{d}(1 - r) + 0.4 r} = \frac{0.4 d}{p n + 0.4d - p}
        \end{align}
    \end{proof}
\end{theorem}

\subsubsection{Preservation of Tendency toward Diagonality}\label{sec:preservation}

\cref{sec:sparsity_at_initialization} has discussed the tendency towards sparsity at initialization, but how this tendency is preserved during training, where $K^l$ and $M^l$ are altered, is still unclear. Since $M^l$'s being moderate is ensured by architectural low-rankness and positive semi-definiteness even in the worst case, we only discuss how diagonality of $K^l \left(K^l\right)^\transpose$ is preserved. We reluctantly make this subsection informal and intuitive because the iterated forward and backward propagation are too complex for analysis.

Inspired by \citet{freq_bias}, we use lazy factors to explain little change in $K^l \left(K^l\right)^\transpose$. In one word, overparameterization and gradient clipping, combined together, amortize the changes across massive parameters, each of which is only slightly changed.

To be more specific, we informally analyze the ``average'' parameter change during training of ViT-Base, which is experimented with by \citet{observation}, under gradient clipping at global norm $1$. Since modern initialization initializes rows approximately to norm $p$, and $K^l \left(K^l\right)^\transpose$ comprises of inner products of rows, we consider a row to be a unit of parameter change. ViT-Base \citep{vit} has in total $12 \times 2$ linear layers, each with 3072 rows, which means each row has to compete for changes with at least $12 \times 2 \times 3072$ rows, letting alone other parameters in position embeddings, biases and MLP layers at self-attention modules. To make that worse, the global norm of gradient in each step is clipped to $1$, making the squared norm of projection from the gradient to the subspace of a row is averagely
\begin{align}
    \frac{1^2}{12 \times 2 \times 3072},
\end{align}
or equivalently the norm of averagely projected gradient is
\begin{align}
    \sqrt{\frac{1^2}{12 \times 2 \times 3072}}.
\end{align}
To make things worse, the learning rate is small. Even under modern practice of large step where batch size and learning rate are both increased, the maximum learning rate is still $\sim 10^{-3}$. Further considering the learning rate scheduling such as Cosine annealing, the average learning rate is about half of the maximum one, which makes the average change as small as
\begin{align}
    \sqrt{\frac{1^2}{12 \times 2 \times 3072}} \times \frac{10^{-3}}{2}.
\end{align}
With this step size, to make an initially unit vector to zero requires $\sqrt{12 \times 2 \times 3072}\times 2 \times 10^3 \approx 5.43 \times 10^5$ steps, while aligning two initially orthogonal unit vectors along the shortest path requires at least $\frac{\sqrt{2}}{2} \approx 0.707$ times of that. With batch size of $512$, the former is equivalent to $217.2$ epochs of ImageNet-1K. For comparison, the PyTorch's recipe trains ViT-Base on ImageNet1k for 300 epochs. As a result, the diagonality will retain for a long time during training.

We argue this informal averaging analysis indeed provide some insights, at least in situations without weight decay. If adaptive optimizers, such as Adam and AdamW, are adopted, they indeed balance the changes among parameters. Moreover, this averaging analysis accounts for a worst case. If more is projected to fewer parameters, then it will be more likely absorbed in $M^l$, which is always moderate by \cref{lemma:ml_diagonality}, and leave a more diagonal $K^l \left(K^l\right)^\transpose$. In experiments we observe that more norm of the gradient concentrate at deeper layers, which is indeed absorbed by $M^l$ of shallow layers.

When it comes to the norm of $K^l$ and $M^l$, we need to deal with weight decay which dramatically reduces the norm of $K^l$ and $M^l$. 
We consider normalization layers, such as BatchNorm and LayerNorm, are saviors for this reduction. If applied before activation, they make weights scale-invariant and introduce some effective weights, which always have moderate norms. The interaction between weight decay and normalization in the context of sparsity and diagonality requires further analysis.


\subsubsection{Reflecting on Diagonality and its Preservation}\label{sec:reflection}

\cref{theorem:diagonality_at_initialization} establishes the relation between diagonality and initialization. The diagonality depends on the ratio $d / n$, and the initialization distribution of entries. When $d/n$ is large enough, this explanation suits perfectly.
However, it does not apply to current actual scenarios because 1) $d/n$ is small, for example in ViT-Base $d/n=768/3072=1/4$, and can be even smaller for larger models; and 2) weights are usually initialized with uniform distribution instead of Gaussian, for example in ViT-Base's recipe by PyTorch \citep{pytorch_recipe}. 
On the other hand, weight decay, if applied, reduces the norm of parameters rapidly, or enlarges the effective learning rate \citep{zhang_three_2018}, endangering lazy diagonality preservation of $\kkT$. 
These inapplicablities are verified by experiments in \cref{sec:t_experiments}, where initial non-diagonal elements have total norm hundreds of times than diagonal ones.
We propose in \cref{sec:spectral} another spectral initial explanation that applies better to cases where $d / n$ is small and initialization is based on uniform distribution. Some assumptions are made, but they are supported by evidences in \cref{sec:t_experiments}.

However, this failed explanation hints potential improvements. This implies that if an initialization distribution that makes $\inner{K^l_i}{K^l_j}$ concentrate better than Gaussian is proposed, we can potentially improve the gradient sparsity. It is also beneficial to use wider weights where $d$ is larger than $n$. This, on the other hand, also allows rows in $K^l$ to be mutually orthogonal and permits perfect sparsity, which is impossible when $n > d$. This modification is referred to as wide MLP.



\appendix


\section{Proof of Lemmas and Corollaries}\label{appendix:proof_of_lemmas}

\begin{proof}[Proof of \cref{lemma:KKT_diagonality_at_initialization}]\label{proof:kkt_diagonality_at_initialization}
    Xavier or Kaiming initialization generate independently $\gaussian{0}{\frac{p}{d}}$-distributed entries in $K^l$ such that the variances of weights for each neuron, i.e., entries in each row, sum to $p$. This translates to 
    \begin{align}
        \sum_k \var{K^l_{i, k}}
        =&  \sum_k \ex{\left(K^l_{i, k} - \ex{K^l_{i, k}}\right)^2} = \sum_{k} \ex{\left(K^l_{i, k}\right)^2} \\
        =&  \ex{\norm{K^l_i}_2^2} = p.
    \end{align}
    Moreover, since $\norm{K^l_i}_2^2 = \sum_{k} \left(K^l_{i, k}\right)^2$ is the sum of squared Gaussian random variables scaled by $\frac{\sqrt{p}}{\sqrt{d}}$, it is subjected to scaled Chi-squared distribution $\frac{p}{d} \chisquared{d}$.
    The CDF of it is \citep{chi_squared}
    \begin{align}
        F(x) = F_{\chisquared{d}}\left(\frac{x d}{p}\right) = \frac{1}{\Gamma\left(\frac{d}{2}\right)} \gamma\left( \frac{d}{2}, \frac{x d}{2 p} \right).
    \end{align}
    By Stirling's approximation there is $\Gamma(a) \sim \sqrt{2 \pi (a - 1)} \left(\frac{a-1}{e}\right)^{a-1}$, while there is $\gamma(a, z) = \frac{e^{-z}z^a}{a} \left[ 1 + O\left(\frac{z}{a}\right)\right]$ \citep{asymptotic_incomplete_gamma}. So given that $\frac{z}{a}$ is $O(1)$, the fraction is asymptotically
    \begin{align}
        \frac{\gamma(a, z)}{\Gamma(a)}
        \sim&   \frac{\frac{e^{-z} z^a}{a}}{\sqrt{2 \pi (a-1)} \left(\frac{a-1}{e}\right)^{a-1}}\\
        \le&  \frac{1}{\sqrt{2 \pi (a-1)}} e^{a + 1 - z} \left(\frac{z}{a-1}\right)^a\\
        \le&  \frac{1}{\sqrt{2 \pi (a-1)}} \left(e^{1 + \frac{1 - z}{a}}\frac{z}{a-1}\right)^a\\
    \end{align}
    So it is sufficient to force $e^{1 + \frac{1 - z}{a}} \frac{z}{a-1} < 1 \iff 1 + \frac{1 - z}{a} + \ln \frac{z}{a - 1} < 0$ in order to ensure the exponential decay of $F(x)$ w.r.t. $a = \frac{d}{2}$.
    \begin{align}
        1 + \frac{1-z}{a} + \ln\frac{z}{a-1}
        =&  \ln \frac{z}{a} - \frac{z}{a} + 1 + \frac{1}{a} + \ln \frac{a}{a-1}\\
        \le&  \ln \frac{z}{a} - \frac{z}{a} + 1 + \frac{1}{a} + \frac{1}{a - 1}\\
        \le&  \ln \frac{z}{a} - \frac{z}{a} + 1 + \frac{2}{a - 1}
    \end{align}
    Since for any $x > 0$ there is $\ln x \le x - 1$, there is $\ln \frac{z}{a} - \frac{z}{a} + 1 \le 0$. Since $\frac{2}{a-1}$ can be arbitrarily small, when $a$ scales sufficiently large with $d$, for any constant $x = O(1)$ such that $\frac{z}{a} = \frac{x}{p} \neq 1$, $F(x)$ drops exponentially as $d$ increases.

    We numerically compute the probability of $\inner{K^l_i}{K^l_i} < p \cdot x$ when $d = 100$ with the following Mathematica codes,
    \lstset{
        basicstyle=\ttfamily
    }
    \begin{lstlisting}
        ScaledChi2CDF[d_, x_] := CDF[ChiSquareDistribution[d], d*x];
        N[ScaledChi2CDF[100, #]] & /@ {0.1, 0.5, 0.7, 0.9, 0.99, 0.999}
    \end{lstlisting}
    which outputs $\{2.18106 \times 10^{-32}, 6.95331 \times 10^{-6}, 0.0098455, 0.246802, 0.490528, 0.515991\}$.

    Now turn to non-diagonal elements. Supposing $i \neq j$, there is 
    \begin{align}
        \ex{\inner{K^l_i}{K^l_j}}
        =&  \inner{\ex{K^l_i}}{\ex{K^l_j}}  &   \left(\text{independence}\right)\\
        =&  \inner{0}{0} = 0.   &   \left(\text{centered}\right)
    \end{align}
    To see how well these inner products concentrate, we calculate their variance. According to \citep{product_of_gaussian}, there is
    \begin{align}
        \inner{K^l_i}{K^l_j}
        =&  \sum_{k} K^l_i K^l_j = \sum_{k}\frac{1}{4}\left(\left(K^l_i + K^l_j\right)^2 - \left(K^l_i - K^l_j\right)^2\right)\\
        =&  \sum_k \left(\frac{\var{K^l_i + K^l_j}}{4} Q_k - \frac{\var{K^l_i - K^l_j}}{4} R_k\right)\\
        =&  \frac{p}{2 d}(Q - R),
    \end{align}
    where $Q_k, R_k \sim \chisquared{1}$ is mutually independent since $K^l_i$ and $K^l_j$ have the same variance, and $Q, R \sim \chisquared{d}$. Since the variance of Chi-squared distribution of freedom $d$ is $2d$ \citep{chi_squared}, the variance of non-diagonal elements is
    \begin{align}
        \var{\inner{K^l_i}{K^l_j}}
        =&  \left(\frac{p}{2d}\right)^2 \left(\var{Q} + \var{R}\right) = \frac{p}{d}.
    \end{align}
    The expectation of the squared inner product is the same as the variance becuase the inner product is centered.

\end{proof}



\subsection{Inapplicability of Diagonal Explanation}

To show the diagonality of $\kkT$ is lost during training, the $L_1$ norm and/or squared $L_2$ norm ratios of diagonal elements and non-diagonal elements are computed. To ease presentation, they are displayed in \cref{fig:diagonal} after being taken $\log_{10}$.

\begin{figure}
    \addvalue{norm1}{$L_1$}
    \addvalue{norm2}{Squared $L_2$}
    \centering
    \foreach \norm in {1, 2}{
        \begin{subfigure}[t]{0.29\textwidth}
            \centering
            \includegraphics[width=\textwidth]{pic/results/dumps/imagenet1k/sparsified/diagonal/ratio_norm\norm_kkT.jpg}
            \caption{\scriptsize \usevalue{norm\norm} norm ratio.}\label{fig:diagonal_norm\norm}
        \end{subfigure}
    }
    \begin{subfigure}[t]{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pic/results/dumps/imagenet1k/sparsified/from_scratch4/4_7_8_10.jpg}
        \caption{\scriptsize Training sparsity of Layer 5, 8, 9 and 11.}\label{fig:pruned_layers}
    \end{subfigure}
    \caption{The $L_1$ and/or squared $L_2$ norm ratio between diagonal and non-diagonal elements of $\kkT$ at early stage, when modified ViT-Base is trained from scratch on ImageNet-1K.}\label{fig:diagonal}
\end{figure}

It can be seen from \cref{fig:diagonal}, especially diagonality measured by squared $L_2$ norm in \cref{fig:diagonal_norm2}, that the diagonality is initialized well as proved in \cref{theorem:diagonality_at_initialization}. However, this diagonality is quickly lost after several steps, possibly due to weight decay. There are also drastic drops at Layer 5, 8, 9 and 11. \cref{fig:pruned_layers} indicates that these layers are entirely pruned, right slightly before these drops. After zero activation, back propagated gradients are also zeroed, leaving them solely to weight decay and quickly become zero matrices and behaves strangely in terms of norm ratio in \cref{fig:diagonal_norm1} and \cref{fig:diagonal_norm2}. So diagonality drops in Layer 5, 8, 9 and 11 somehow do not really count. The rest significantly drops but recovers in later steps. Despite this recovering, the lazy and inert diagonal explanation based on gradient amortization still fails under weight decay because otherwise diagonalities should have not dropped at the first several steps. \cref{fig:diagonal_norm2} indicates some more dynamic factors are encouraging diagonality recovering, which spectral explanation, as an extension to the diagonal one, can embrace.

Further result is left in later version, because previous experiments are based on even former theories and did not observe diagonalities.

==> failed/loose-bounds.tex <==
\begin{lemma}[Bounds of on \sti{} transform]\label{lemma:bound_of_sti_old}
    Suppose $S \in \complexes$ satisfies 
    \begin{align}
        \frac{S}{1 + S} - z S = c + t,
    \end{align}
    where $z = 0 + v i \in \positivecomplex (v \in \reals^+), c \in \reals^+, t \in \complexes$, then
    \begin{align}
        \abs{\ipart{S}} \le \abs{S} \le&  \frac{2}{v} \left(c + \abs{t} + v + 1\right)^2 + 4 \left(c + \abs{t}\right).
    \end{align}
\end{lemma}
\begin{proof}
    $S$ is either
    \begin{align}
        S_1 = -\frac{-\sqrt{(-c-t-z+1)^2+4 z (-c-t)}+c+t+z-1}{2 z}
    \end{align}
    or
    \begin{align}
        S_2 = -\frac{\sqrt{(-c-t-z+1)^2+4 z (-c-t)}+c+t+z-1}{2 z},
    \end{align}
    both of which, since $z = v i, v \in \reals^+$, satisfy
    \begin{align}
        \abs{S} 
        \le&
            \frac{1}{v} \left(
                1 + v + \abs{t} + c + \abs{(-c-t-z+1)^2+4 z (-c-t)}
            \right)\\
        \le&
            \frac{1}{v} \left(
                1 + v + \abs{t} + c + \abs{-c-t-z+1}^2 + 4 v \abs{-c-t}
            \right)\\
        \le&
            \frac{1}{v} \left(
                1 + v + \abs{t} + c + \left(c + \abs{t} + v + 1\right)^2 + 4 v \left(c + \abs{t}\right)
            \right)\\
        \le&  \frac{2}{v} \left(c + \abs{t} + v + 1\right)^2 + 4 \left(c + \abs{t}\right).
    \end{align}
\end{proof}

==> failed/mp-in-batch.tex <==
Assuming batch sampling with replacement (which slightly diverges common practice of sampling without replacement), columns in $\Eta^t$ or $X^t$ are mutually independent, but there can be dependence within one column. To adapt to it, we rely an extension of Marchenko-Pastur distribution under dependence within independent columns proved in \citep{mp_quadratic_form}.
\begin{theorem}[Marchenko-Pastur distribution, extended under column dependence \citep{mp_quadratic_form}]\label{theorem:ext_mp_distribution}
    Let $X^{p, b} \in \reals^{p \times b}$ be a random matrix whose columns $X^{p, b}_{\cdot, j} \in \reals^{p}$ are I.I.D. copies of some random vector $x^p \in \reals^{p}$ for all $p, b \ge 1$.

    If $\left(\left(x^p\right)^\transpose A^p x^p - \trace{A^p}\right) / p \xrightarrow{p} 0$ as $p \to \infty$ for all sequences of $p \times p$ complex matrices $A^p$ with uniformly bounded spectral norms $\norm{A^p}$, then with probability $1$, empirical spectral density of $\frac{1}{b} X^{p, b} \left(X^{p, b}\right)^\transpose$ is weakly convergent to Marchenko-Pastur distribution as $p \to \infty$ with $p / b \to c$.
\end{theorem}
We develop a sufficient condition suitable for $\Eta$ and $U$ in \cref{corollary:spectral_of_single_step}.
\begin{restatable}[Spectral property of single step]{corollary}{SpectralOfSingleStep}
    \label{corollary:spectral_of_single_step}

    Inherit notation defined in \cref{theorem:ext_mp_distribution}. Particularly, the columns in $X^p$ are independent.
    Let $S^p \defeq \ex{x^p \left(x^p\right)^\transpose}$ be the covariance matrix of the random vector at $p$, and $I_p$ be the compatible identity matrix.
    Assume $x^p$'s norm is bounded, say by $1$, and scale it with 
    \begin{align}
        u^p \defeq \sqrt{\alpha} x^p,
    \end{align}
    where $\alpha \defeq \frac{\trace{S^p}}{\trace{S^p S^p}}$. Let $T^p \defeq \ex{u^p \left(u^p\right)^\transpose} = \alpha \cdot S^p$ be the covariance matrix of $u^p$. Let $U^p \in \reals^{p \times b}$ be the matrix consisting of I.I.D. copies of $u^p$.

    If $\trace{(T^p - I^p)(T^p - I^p)} / p \to 0$ and $\alpha / p \to 0$, then with probability $1$, empirical spectral density of $\frac{1}{b} U^p \left(U^p\right)^\transpose$ weakly converges to Marchenko-Pastur distribution as $p \to \infty$ with $p / b \to c$.
\end{restatable}

Its proof is left in \cref{appendix:proof_of_lemmas}. To apply \cref{corollary:spectral_of_single_step} on $\Eta^t \left(\Eta^t\right)^\transpose$ and $X^t \left(X^t\right)^\transpose$, we empirically verify that $\trace{(T^p - I^p)(T^p - I^p)} = o(p)$ and $\alpha = o(p)$ of both back-propagated gradients $\eta^{l, s}$ and inputs $u^{l, s}$ to the weight for the entire training set $\dataset$. Since hidden dimension must be altered multiple times, it is done on small data set MNIST using LayerNorm-ed (features are bounded) tiny pure MLP or a tiny ViT. It is observed that the two statistics increase in a rate much slower than the increase of hidden dimension, at least when dimension is about several hundred. Therefore we consider \cref{corollary:spectral_of_single_step} approximately applicable to real scenarios. Therefore, non-zero eigenvalues in $\Eta^t \left(\Eta^t\right)^\transpose$ and $X^t \left(X^t\right)^\transpose$ concentrate in a extremely narrow interval, compared to their distance to $0$.
\SpectralOfSingleStep*
\begin{proof}[Proof of \cref{corollary:spectral_of_single_step}]
    We first prove that expectation of $\utau$ converges to $\trace{A^p}$ with rate $o(p)$, and then show the its variance converges to $0$ at rate $o(p^2)$. If both claim is done, then for every $\epsilon > 0$
    \begin{align}
        &   \lim_{p \to \infty} \prob{\abs{\left(\utau - \trace{A^p} \right) / p - 0} > \epsilon}\\
        \le&    \lim_{p \to \infty} \prob{
                \abs{\utau - \ex{\utau}} / p
                + \abs{\ex{\utau} - \trace{A^p}} / p >
            \epsilon}\\
        =&    \lim_{p \to \infty} \prob{
                \abs{\utau - \ex{\utau}} / p >
            \epsilon}\\
        &   \left(\text{Chebyshev's inequality}\right)\\
        \le&    \lim_{p \to \infty} \frac{\var{\utau}}{p^2 \epsilon^2} = 0,
    \end{align}
    and the weak convergence is proved.

    For the asymptotic unbiasedness, when $p$ is sufficiently large to use $\norm{A_p}$'s uniform bound,
    \begin{align}
        \abs{\frac{\ex{\utau} - \trace{A^p}}{p}}\label{eq:p_convergence_start}
        =&  \frac{\abs{\trace{\left(\ex{\uut} - I^p\right)^\transpose A^p}}}{p}\\
        % &   \left(\abs{\sum_{i} \lambda_i} \le \sum_{i} \abs{\lambda_i} \right)\\
        \le&    \frac{\norm{\left(T^p - I^p\right)^\transpose A^p}_1}{p}\\
        &   \left(\text{Hölder's inequality, applied on absolute singular values}\right)\\
        \le&    \frac{\norm{T^p - I^p}_1 \norm{A_p}_{\infty}}{p}\\
        &   \left(\text{spectral norms $\norm{A^p} = \norm{A^p}_{\infty}$ are uniformly bounded}\right)\\
        \le&    O(1) \cdot \frac{\norm{T^p - I^p}_1}{p},
    \end{align}
    where $\norm{\cdot}_k$ indicates Schatten $k$-norms, i.e., $L_k$ norms taken on singular values. To continue, only focusing on $\frac{\norm{T^p - I^p}}{p}$ gives
    \begin{align}
        \frac{\norm{T^p - I^p}_1}{p}
        \le&    \frac{\sqrt{p} \norm{T^p - I^p}_2}{p} \label{step:upperbound_L1_by_L2}\\
        =&      \sqrt{\trace{\left(T^p - I^p\right)^\transpose \left(T^p - I^p\right)} / p},
    \end{align}
    where \cref{step:upperbound_L1_by_L2} follows the upperbound of $L_1$ norm by $L_2$ norm.
    By condition $\trace{(T^p - I^p)(T^p - I^p)} / p \to 0$, 
    \begin{align}
        \abs{\frac{\ex{\utau} - \trace{A^p}}{p}}
        \le&    O(1) \cdot \sqrt{\trace{\left(T^p - I^p\right)^\transpose \left(T^p - I^p\right)} / p} \to 0.
    \end{align}

    For variance's diminishment, 
    \begin{align}
        \var{\utau}
        =&  \ex{\trace{\utau \utau}} - \ex{\trace{\utau}}^2 \label{eq:p_convergence_variance_begin}\\
        =&  \alpha^2 \left(\ex{\trace{\xtax \xtax}} - \ex{\trace{\xtax}}^2\right)\\
        \le&    \alpha^2 \ex{\trace{\xtax \xtax}}   \le    \alpha^2 \ex{\norm{x^p}_2^4 \norm{A}^2}\\
        =&  \alpha^2 \cdot O(1),\label{eq:p_convergence_end}
    \end{align}
    where the last step follows that $x^p$'s norm is bounded and that $\norm{A}$ is also uniformly bounded. Since $\alpha = o(p)$, $\var{\utau} = o(p^2)$.

    To gave a scaling factor $\alpha$ encouraging best convergence, minimize the difference bound of $\ex{\utau}$ and $\trace{A^p}$ proved before, i.e.
    \begin{align}
        \trace{\left(T^p - I^p\right)^\transpose \left(T^p - I^p\right)}
        =&  \trace{\left(\alpha S^p - I^p\right)^\transpose \left(\alpha S^p - I^p\right)}
    \end{align}
    whose derivative w.r.t. $\alpha$ is $\trace{S^p \left(\alpha S^p - I^p\right)}$. Setting the derivative to $0$ gives
    \begin{align}
        \trace{S^p \alpha S^p} =^ \trace{S^p}\\
        \alpha = \frac{\trace{S^p}}{\trace{S^p S^p}}.
    \end{align}
\end{proof}

==> failed/post-eff.tex <==
To exploit the eigenvalue concentration, we define effective sparsity in \cref{def:effective_gradient_sparsity} following \cref{lemma:rewrite_gradient_sparsity}.
\begin{lemma}\label{lemma:rewrite_gradient_sparsity}
    Let $g^l \defeq \left(J_{\ce}(f) J_f(\dbmlp^l)\right)^\transpose \in \reals^{n}$ be the (column) gradient w.r.t. activations of $\mlp^l$ or $\dbmlp^l$, then there is $M^l = g^l \left(g^l\right)^\transpose$. Furthermore, we have
    \begin{align}
        \left(\gamma^l\right)^\transpose \left(\left(K^l \left(K^l\right)^\transpose\right) \hadamard M^l\right) \gamma^l
        =& \left(g^l \hadamard \gamma^l\right)^\transpose \kkT (g^l \hadamard \gamma^l).
    \end{align}
    \begin{proof}
        $M^l = g^l \left(g^l\right)^\transpose$ is straightforward by definition. For the other equality, combining $\diag{\gamma}$ in a way other than what is done in \cref{lemma:adversarial_and_sparsity} gives
        \begin{align}
            &   \left(\gamma^l\right)^\transpose \left(\left(K^l \left(K^l\right)^\transpose\right) \hadamard M^l\right) \gamma^l\\
            =&  \left(\gamma^l\right)^\transpose \diag{g^l} \kkT \diag{g^l} \gamma^l\\
            =& \left(g^l \hadamard \gamma^l\right)^\transpose \kkT (g^l \hadamard \gamma^l).
        \end{align}
    \end{proof}
\end{lemma}


==> theory/proof0.tex <==
The proof is adapted from \citet{mp_quadratic_form} where independence condition is replaced with new regularities.


Cauchy-\sti{} transform method is used. 
For completeness, \sti{} transform of a distribution $\mu$ is 
\begin{align}
    s^\mu(z) \defeq \int_{\reals} \frac{1}{\lambda - z} \mu(\dd \lambda), \forall z \in \positivecomplex,
\end{align}
where $\positivecomplex \defeq \set{u + v i: u, v \in \reals, v > 0} \subset \complexes$.
When applied to empirical spectral density, by definition there is
\begin{align}
    s^{F^A}(z) = \trace{A - z I}^{-1} / p \defeq \trace{\left(A - z I\right)^{-1}} / p.
\end{align}
for positive semi-definite $A \in \reals^{p \times p}$.
Specifically $\frac{1}{b T} U^p \left(U^p\right)^\transpose = \frac{1}{b T} U U^\transpose$'s \sti{} transform is
\begin{align}
    s_p(z) = \trace{\frac{1}{b T} U U^\transpose - z I}^{-1} / p = b T / p \trace{U U^\transpose - z b T I}.
\end{align}
By \sti{} continuity theorem \citep{RMT_book}, it is sufficient to show that $s_p(s) \asto s(z)$ for all $z \in \positivecomplex$, where $s$ is the \sti{} transform of Marchenko-Pastur distribution with parameter $p$ and $n$. To this end, typical steps include the following steps \citep{mp_proof_sketch}:
\begin{itemize}
    \item $s_p(z) - \ex{s_p(z)} \asto 0$, by a martingale argument;
    \item $\ex{s_p(z)} \to s(z)$.
\end{itemize}

Before we start, a handy lemma proved by \citet{mp_quadratic_form} is repeated.
\begin{lemma}[\citep[][Lemma 3.1]{mp_quadratic_form}]\label{lemma:3.1_from_mp_quadratic_form}
    Let $C \in \reals^{p \times p}$ be a real symmetric positive semi-definite matrix and $x \in \reals^p$. If $z \in \complexes$ is such that $v = \ipart{z} > 0$, then
    \begin{enumerate}
        \item\label{lemma:spectral_bound_of_reverse} 
            $\norm{\left(C - z I\right)^{-1}} \le 1 / v$ ;
        \item\label{lemma:x_means_little_in_reversed_sample_covariance}
            $\abs{\trace{C + x x^\transpose - z I}^{-1} - \trace{C - z I}^{-1}} \le 1 / v$;
        \item $\abs{x^\transpose\left(C + x x^\transpose - z I\right)^{-1} x} \le 1 + \abs{z} / v$;
        \item $\ipart{z + z \trace{C - z I}^{-1}} \ge v$ and $\ipart{\trace{C - z I}^{-1}} > 0$;
        \item $\ipart{z + z x^\transpose (C - z I)^{-1} x} \ge v$.
    \end{enumerate}
\end{lemma}

For $s_p(z) - \ex{s_p(z)}$'s almost sure convergence, \citet{mp_quadratic_form} refer to \citet{mp_proof_sketch}, which we will repeat here to examine and replace independence assumptions within.

\NewDocumentCommand{\condiex}{O{k} m}{\ex[#1]{#2}}
Let $\condiex[k]{\cdot} \defeq \ex{\cdot \mid U^p_{\cdot, 1: k}}$ denote the conditional expectation given $U^p_{\cdot, 1}, \dots, U^p_{\cdot, k}$. Then $s_p(z) = \condiex[b]{s_p(z)}$ and $\ex{s_p(z)} = \condiex[0]{s_p(z)}$, and there is
\begin{align}
    s_p(z) - \ex{s_p(z)}
    =&  \sum_{k=1}^{b} \left(\condiex[k]{s_p(z)} - \condiex[k-1]{s_p(z)}\right)
    =  \sum_{k=1}^{b} \gamma_k,
\end{align}
where $\gamma_k \defeq \condiex[k]{s_p(z)} - \condiex[k-1]{s_p(z)}$. Note that $\set{\condiex[k]{s_p(z)}}_k$ is already a Doob martingale, so $\set{\gamma_k}_k$, as its difference, is a sequence of martingale differences.
        
\NewDocumentCommand{\invC}{O{1}}{\left(C^p_k\right)^{-#1}}
Let $C^p_{k} \defeq \frac{1}{b T} \sum_{k'} \uut[k'] - z I - \frac{1}{b T}u_k u_k^\transpose$. By \cref{lemma:3.1_from_mp_quadratic_form}(1), $C^p_{k}$ is invertible, and by Sherman-Morrison formula there is
\begin{align}
    s_p(z)
    =&  \trace{C^p_k + \frac{1}{b T} u_k u_k^\transpose }^{-1} / p
    =  \frac{1}{p} \trace{\invC - \frac{\invC u_k u_k^\transpose \invC / b T}{1 + u_k^\transpose \invC u_k / b T}}\\
    =&  \frac{1}{p} \left(\trace{\invC} - \frac{u_k^\transpose \invC[2] u_k}{b T + u_k^\transpose \invC u_k}\right).
\end{align}
Since $u_k$ is not involved in $C^p_k$, $\condiex[k]{\trace{\invC}} = \condiex[k-1]{\trace{\invC}}$. Regarding the second term,
\begin{align}
    &   \abs{\frac{u_k^\transpose \invC[2] u_k}{b T + u_k^\transpose \invC u_k}}\\
    =&      \frac{\abs{\trace{u_k u_k^T \invC \invC}}}{\abs{b T + u_k^\transpose \invC u_k}}
    \le    \frac{\norm{u_k u_k^T \invC \invC}_1}{b T + u_k^\transpose \invC u_k}\\
    \le&   \frac{\norm{u_k u_k^T \invC}_1 \norm{\invC}_{\infty}}{b T + u_k^\transpose \invC u_k}
    \le    \frac{1}{v} \frac{u_k^T \invC u_k}{b T + u_k^\transpose \invC u_k}
    \le \frac{1}{v},
\end{align}
where the second inequality follows \cref{lemma:3.1_from_mp_quadratic_form}(1).
Therefore $\gamma_k$ can be bounded by
\begin{align}
    \gamma_k \le& \frac{2}{v} \frac{1}{p}.
\end{align}
By Azuma's inequality, there is
\begin{align}
    \prob{\abs{s_p(z) - \ex{s_p(z)}} > \epsilon} \le 2 \exp\left(-\frac{\epsilon^2}{2 p \left(\frac{2}{v} \frac{1}{p}\right)^2}\right) \le 2 \exp\left(-\epsilon^2 v^2 p / 8\right).
\end{align}
Given that $\prob{\abs{s_p(z) - \ex{s_p(z)}}}$ decays exponentially with $p$, for every $\epsilon > 0$, there is
\begin{align}
    \sum_{p=0}^\infty \prob{\abs{s_p(z) - \ex{s_p(z)}} > \epsilon} < \infty
\end{align}
which implies $s_p(z) - \ex{s_p(z)} \asto 0$ \citep[see][Theorem 7.5]{exponential_decay_to_as}.

We adapt proof of Theorem 2.1 by \citet{mp_quadratic_form} to check $\ex{s_p(z)} \to \ex{s(z)}$. 
Define $A^p \defeq \sum_{k} \uut$.
Sample an auxiliary vector $u_{T, b+1} = u_{b T  + 1} \in \reals^p$ so that it is sampled from the conditional distribution given the first $T-1$ batches but it is conditionally independent with other samples in $U^T$, i.e., an extra sample for the last batch. This dependence relation can be expressed by only adding edges $U^{1: T-1} \to u_{T, b+1}$ to the Bayesian network. With the auxiliary vector, define $B^p \defeq A^p +  \uut[T, b+1]$. %Define $C^b_t \defeq B^p - u^t \left(u^t\right)^\transpose$

By \cref{lemma:3.1_from_mp_quadratic_form}(1), $B^p - z b T I$ is non-degenerate and
\begin{align}
    p 
    =&  \trace{\left(B^p - z b T I\right) \left(B^p - z b T I\right)^{-1}}\\
    =&   \sum_{t=1}^{T} \sum_{l=1}^{b + \indic{t = T}} u_{t, l}^\transpose \left(B^p - z b T I\right)^{-1} u_{t, l} - z b T \trace{B^p - z b T I}^{-1}.
\end{align}
Taking expectation and using the exchangeability within a batch give
\begin{align}
    p = \sum_{t=1}^{T} (b + \indic{t = T}) \ex{u_t^\transpose \left(B^p - z b T I\right)^{-1} u_t} - z b T \ex{\trace{B^p - z b T I}^{-1}} \label{eq:a3}.
\end{align}

Independently sample $r_k$ based on $U$ by uniformly randomly selecting one $u_k$ in all $b T + 1$ of them. This leads to
\begin{align}
    &   \frac{1}{b T + 1}\sum_{l} \ex{f(r_l) \times g(U, u_{b T + 1})}\\
    =&  \frac{1}{b T + 1} \sum_{l} \ex{\ex{f(r_l) \times g(U, u_{b T + 1}) \mid U}}
    =  \frac{1}{b T + 1} \sum_{l} \ex{\ex{f(r_l) \mid U} \ex{g(U) \mid U}}\\
    =&  \frac{1}{b T + 1} \sum_{l} \ex{\left(\frac{1}{b T + 1}\sum_{o} f(u_o)\right)\ex{g(U) \mid U}}
    =   \frac{1}{b T + 1} \sum_{o} \ex{f(u_o) \ex{g(U) \mid U}}\\
    =&  \frac{1}{b T + 1} \sum_{o} \ex{\ex{f(u_o) g(U) \mid U}}
    =  \frac{1}{b T + 1} \sum_{o} \ex{f(u_o) g(U)}.
\end{align}
This construction reduces \cref{eq:a3} to \begin{align}
    p = \ex{r \left(B^p - z b T I\right)^{-1} r} - z b T \ex{\trace{B^p - z b T I}^{-1}}.
\end{align}

Define $S_p(z) \defeq \trace{A^p - z b T I}^{-1}$ and note that $S_p(z) = (p / b T) s_p(z)$. 

By \cref{lemma:3.1_from_mp_quadratic_form}(2)-(3), there are
\begin{align}
    \ex{\trace{B^p - z b T I}^{-1}} =& \ex{S_p(z)} + O(1/b T) \label{eq:a1},\\
    \ex{u_t \left(B^p - z b T I\right)^{-1} u_t} =& O(1) \label{eq:a2}.
\end{align}

We now prove,
\begin{align}
    \frac{1}{T} \sum_{t=1}^{T} \ex{u_t^\transpose \left(B^p - z b T I\right)^{-1} u_t} = \frac{\ex{S_p(z)}}{1 + \ex{S_p(z)}} + o(1). \label{eq:claim}
\end{align}
\begin{align}
    \ex{r^\transpose \left(B^p - z b T I\right)^{-1} r} = \frac{\ex{S_p(z)}}{1 + \ex{S_p(z)}} + o(1). \label{eq:claim}
\end{align}
By \cref{lemma:3.1_from_mp_quadratic_form}, $\norm{\left(A^p - z b T I\right)^{-1}} \le \frac{1}{v b T}$ and $\norm{b T\left(A^p - z b T I\right)^{-1}}  \le \frac{1}{v}$. So let $D \defeq b T \left(A^p - z b T I\right)^{-1}$ be the random variable with spectral norm bound $\frac{1}{v}$. Note that $S_p(z) = \trace{D}$ so in the following we shall focus on $\ex{\trace{D}}$. We now repeat steps in \cref{eq:p_convergence_start}-\cref{eq:p_convergence_end} to prove that $\frac{1}{T} \sum_{t=1}^{T}u_t^\transpose D u_t - \ex{\trace{D}} \xrightarrow{p} 0$.
As before, first we prove the convergence of the expectation
\begin{align}
    &       \abs{\ex{\frac{1}{T} \sum_{t=1}^T u_t^\transpose \left(A^p - z b T I\right)^{-1} u_t} - \ex{S_p(z)}}\\
    \sim&   \frac{\abs{\ex{\frac{1}{T} \sum_{t=1}^T u_t^\transpose b T\left(A^p - z b T I\right)^{-1} u_t} - \ex{b T S_p(z)}}}{p}\\
    =&      \frac{\abs{\frac{1}{T} \sum_{t=1}^T  \ex{u_t^\transpose D u_t} - \ex{\trace{D}}}}{p}
    =      \frac{\abs{\ex{\trace{\left(\frac{1}{T} \sum_{t=1}^T u_t u_t^\transpose - I\right) D}}}}{p}\\
    \le&    \frac{\ex{\norm{\left(\frac{1}{T} \sum_{t=1}^T u_t u_t^\transpose - I\right) D}_1}}{p}
    \le    \frac{\ex{\norm{\left(\frac{1}{T} \sum_{t=1}^T u_t u_t^\transpose - I\right)}_1 \norm{D}_{\infty}}}{p}\\
    \le&    \frac{1}{v}\frac{\ex{\norm{\left(\frac{1}{T} \sum_{t=1}^T u_t u_t^\transpose - I\right)}_1}}{p}
    \le    \frac{1}{v p}  \ex{\sqrt{p \trace{\left(T^p - I\right)^\transpose \left(T^p - I\right)}}}\\
    =&      \frac{1}{v} \ex{\sqrt{\frac{\trace{\left(T^p - I\right)^\transpose \left(T^p - I\right)}}{p}}} \to 0.
\end{align}
\begin{align}
    &       \abs{\ex{r^\transpose \left(A^p - z b T I\right)^{-1} r} - \ex{S_p(z)}}\\
    \sim&   \frac{\abs{\ex{r^\transpose b T\left(A^p - z b T I\right)^{-1} r} - \ex{b T S_p(z)}}}{p}\\
    =&      \frac{\abs{\ex{r^\transpose D r} - \ex{\trace{D}}}}{p}
    =      \frac{\abs{\trace{\ex{\left(r r^\transpose - I\right) D}}}}{p}\\
    \le&    \frac{\ex{\norm{\left(r r^\transpose - I\right) D}_1}}{p}
    \le    \frac{\ex{\norm{\left(r r^\transpose - I\right)}_1 \norm{D}_{\infty}}}{p}\\
    \le&    \frac{1}{v}\frac{\ex{\norm{\left(r r^\transpose - I\right)}_1}}{p}
    \le    \frac{1}{v p}  \ex{\sqrt{p \trace{\left(T^p - I\right)^\transpose \left(T^p - I\right)}}}\\
    =&      \frac{1}{v} \ex{\sqrt{\frac{\trace{\left(T^p - I\right)^\transpose \left(T^p - I\right)}}{p}}} \to 0.
\end{align}
The diminishment of variance is almost direct copies of 

Since $\trace{\left(T^{p, t} - I\right)^\transpose \left(T^{p, t} - I\right)} / p \xrightarrow{p} 0$ for every $t$ and $\alpha^t$ is $o(p)$-bounded, repeating \cref{eq:p_convergence_start}-\cref{eq:p_convergence_end}, which are done by bounds on Schatten norms and are irrelevant to independence or dependence, gives
\begin{align}
    &\abs{u_t^\transpose \left(A^p - z b I\right)^{-1} u_t - S_p(z)}\\
    \sim& \abs{u_t^\transpose b T\left(A^p - z b T I\right)^{-1} u_t - b T\trace{A^p - z b T I}^{-1}} / p\\
    \xrightarrow{p}& 0.
\end{align} 
Combining $S_p(z) - \ex{S_p(z)} = (p / b T) \left(s_p(z) - \ex{s_p(z)}\right) \xrightarrow{p} 0$, there is further
\begin{align}
    &   \abs{u_t^\transpose \left(B^p - z b T I\right)^{-1} u_t - \frac{\ex{S_p(z)}}{1 + \ex{S_p(z)}}}\\
    \xrightarrow{p}& 0,
\end{align}
where the first step is due to Sherman-Morrison formula. We refer readers to \citet{mp_quadratic_form} for details of this convergence and its implication to \cref{eq:claim} since it requires no dependence condition.

With \cref{eq:claim}, \cref{eq:a1} and \cref{eq:a2}, \cref{eq:a3} can be reduced to
\begin{align}
    p =& T (b + O(1)) \left(\frac{\ex{S_p(z)}}{1 + \ex{S_p(x)}} + o(1)\right) - z b T \left(\ex{S_p(z)} + O(1 / b)\right),
\end{align}
and
\begin{align}
    \frac{\ex{S_p(z)}}{1 + \ex{S_p(x)}} - z \ex{S_p(z)} =& \frac{p}{b T} + o(1) = c + o(1).
\end{align}
The final conclusion is reached the same way as \citet{mp_quadratic_form}.
